CVaR-based Safety Analysis in the Infinite Time Horizon Setting

We develop a risk-averse safety analysis method for stochastic systems on discrete infinite time horizons. Our method quantifies the notion of risk for a control system in terms of the severity of a harmful random outcome in a fraction of the worst cases. In contrast, classical methods quantify risk in terms of the probability of a harmful event. Our theoretical arguments are based on the analysis of a value iteration algorithm on an augmented state space. We provide conditions to guarantee the existence of an optimal policy on this space. We illustrate the method numerically using an example from the domain of stormwater management.

==> long_proof_Lemma1.tex <==
\hspace{-7mm}\begin{proof}
Let $\pi = (\mu_0,\mu_1,\dots) \in \Pi'$, $s \in \mathbb{R}$, and $(x,z) \in S \times \mathcal{Z}$ be given. For any $t \in \mathbb{N}_0$, the definition of $J_{t,s}^\pi(x,z)$ is $\int_\Omega \max\{Z_t - s,0\} \mathrm{d}P_{x,z}^\pi$. If $t = 0$, then 
$J_{0,s}^\pi(x,z) = \int_\Omega \max\{Z_0 - s,0\} \mathrm{d}P_{x,z}^\pi = \max\{z - s,0\} = v_0^s(x,z)$ since $Z_0 = z$ everywhere. Now, if $t \in \mathbb{N}$, then
\begin{equation}\label{my99}\begin{aligned}
     Z_t(\omega)  = z_t & = \max\{z_{t-1},c(x_{t-1},u_{t-1})\} \\ &= \max\{z_0,c(x_0,u_0),\dots,c(x_{t-1},u_{t-1})\}
\end{aligned}\end{equation}
for any $\omega = (x_0,z_0,u_0,x_1,z_1,u_1,\dots) \in \Omega$. Recall that $\Omega_{t+1} := (S \times \mathcal{Z} \times C)^{t+1}$, whose elements take the form $\omega_{t+1} = (x_0,z_0,u_0,\dots,x_{t},z_{t},u_{t}) \in \Omega_{t+1}$. It holds that $Z_t : \Omega_{t+1} \rightarrow \mathbb{R}$ is a non-negative Borel-measurable function by \eqref{my99} and because $c$ is Borel measurable and non-negative, $\max$ is Borel measurable, and each $z_0 \in \mathcal{Z}$ is a non-negative real number. 
%In particular, $Z_t$ is constant in the coordinates $(x_t,u_t)$. 
%then $Z_1(\omega) = \max\{z_{0},c(x_{0},u_{0})\}$ for any $\omega \in \Omega$ of the form above, and $Z_1 : \Omega_2 \rightarrow \mathbb{R}$ is Borel measurable, non-negative, and constant in the coordinates $(x_1,u_1)$. 
We use \eqref{marginal} to express $J_{1,s}^\pi(x,z)$ as follows:
\begin{equation}\begin{aligned}
     & J_{1,s}^\pi(x,z)  \\
     & := \textstyle \int_\Omega \max\{Z_1 - s,0\} \; \mathrm{d}P_{x,z}^\pi \\
     & \hphantom{:}= \textstyle \int_{\Omega_2} \max\{Z_1 - s,0\} \; \mathrm{d}P_{x,z}^{\pi,2}\\
     & \hphantom{:}= \textstyle \int_{S} \int_{\mathcal{Z}}\int_C \int_{S} \int_{\mathcal{Z}} \int_C \max\{z_1 - s,0\}
     \mu_{1}(\mathrm{d}u_{1}|x_1,z_1) \\ & \hphantom{:==} \overline{Q}(\mathrm{d}(x_1,z_1)|x_0,z_0,u_{0}) \mu_{0}(\mathrm{d}u_{0}|x_0,z_0)  \nu_{x,z}(\mathrm{d}(x_0,z_0)).
\end{aligned}\end{equation}
Since $\max\{z_1 - s,0\} = v_0^s(x_1,z_1)$ is constant in $(x_1,u_1)$ and by the definitions of $\overline{Q}$, $\nu_{x,z}$ \eqref{2b}, and $T_{\mu_0}$ (Def. \ref{DPoperator}), it follows that
\begin{equation}\begin{aligned}
    J_{1,s}^\pi(x,z)
   & = \textstyle \int_C \int_{S} \int_{\mathcal{Z}}  \max\{z_1 - s,0\}\delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1)
      \\ & \hphantom{:==}  Q(\mathrm{d}x_1|x,u_0) \mu_{0}(\mathrm{d}u_{0}|x,z)  \\
      & = T_{\mu_0}(v_0^s)(x,z).
\end{aligned}\end{equation}
Let $t \in \{2,3,\dots\}$ be given, and we proceed through a similar derivation. We use \eqref{marginal} to express $J_{t,s}^\pi(x,z)$ as follows:
\begin{equation}\begin{aligned}
   &  J_{t,s}^\pi(x,z) \\
   & = \textstyle \int_{\Omega_{t+1}} \max\{Z_{t} - s,0\} \; \mathrm{d}P_{x,z}^{\pi,t+1}\\
   & = \textstyle \int_{S \times \mathcal{Z}}\int_{C} \int_{S\times \mathcal{Z}} \cdots \int_{S \times \mathcal{Z}}\int_C \max\{z_t - s, 0\} \mu_{t}(\mathrm{d}u_{t}|\overline{x}_{t})\\ & \overline{Q}(\mathrm{d}\overline{x}_{t}|\overline{x}_{t-1},u_{t-1}) \cdots \overline{Q}(\mathrm{d}\overline{x}_1|\overline{x}_0,u_{0}) \mu_{0}(\mathrm{d}u_{0}|\overline{x}_0) \nu_{x,z}(\mathrm{d}\overline{x}_0).
\end{aligned}\end{equation}
Since $\max\{z_t - s, 0\} = v_0^s(x_t,z_t)$ is constant in $(x_t,u_t)$ and from the definition of $\overline{Q}$ and $\nu_{x,z}$, it follows that
\begin{equation}\begin{aligned}
    & J_{t,s}^\pi(x,z) \\  & = \textstyle \int_{C} \int_{S} \int_ {\mathcal{Z}} \cdots \Big( \int_{C} \int_{S} \int_{\mathcal{Z}}v_0^s(x_t,z_t) 
   \delta_{\max\{z_{t-1},c(x_{t-1},u_{t-1})\}}(\mathrm{d}z_t)\\ & \hphantom{==} Q(\mathrm{d}x_t|x_{t-1},u_{t-1}) \mu_{t-1}(\mathrm{d}u_{t-1}|x_{t-1},z_{t-1}) \Big) \\ & \hphantom{==} \cdots \delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1)Q(\mathrm{d}x_1|x,u_{0}) \mu_{0}(\mathrm{d}u_{0}|x,z),\\
\end{aligned}\end{equation}
where there are $t$ copies of $C \times S \times \mathcal{Z}$.
The term in parenthesis is $T_{\mu_{t-1}}(v_0^s)(x_{t-1},z_{t-1})$, which allows us to write,
\begin{equation}\label{my14}\begin{aligned}
    & J_{t,s}^\pi(x,z) \\  & = \textstyle \int_{C} \int_{S} \int_ {\mathcal{Z}} \cdots T_{\mu_{t-1}}(v_0^s)(x_{t-1},z_{t-1}) \cdots \delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1) \\ & \hphantom{==} Q(\mathrm{d}x_1|x,u_{0}) \mu_{0}(\mathrm{d}u_{0}|x,z)
\end{aligned}\end{equation}
with $t-1$ copies of $C \times S \times \mathcal{Z}$ in \eqref{my14}. By writing more of the integrals explicitly, we find that
\begin{equation}\begin{aligned}
    & J_{t,s}^\pi(x,z) \\  & = \textstyle \int_{C} \int_{S} \int_ {\mathcal{Z}} \cdots \Big( \int_{C} \int_{S} \int_ {\mathcal{Z}} T_{\mu_{t-1}}(v_0^s)(x_{t-1},z_{t-1}) \\ & \hphantom{==} \delta_{\max\{z_{t-2},c(x_{t-2},u_{t-2})\}}(\mathrm{d}z_{t-1}) Q(\mathrm{d}x_{t-1}|x_{t-2},u_{t-2}) \\ & \hphantom{==} \mu_{t-2}(\mathrm{d}u_{t-2}|x_{t-2},z_{t-2}) \Big) \cdots\\ & \hphantom{==} \delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1)  Q(\mathrm{d}x_1|x,u_{0}) \mu_{0}(\mathrm{d}u_{0}|x,z).
\end{aligned}\end{equation}
The term in the parenthesis is $T_{\mu_{t-2}}\big( T_{\mu_{t-1}}(v_0^s)\big)(x_{t-2},z_{t-2})$ by Def. \ref{DPoperator}, and we obtain
\begin{equation}\label{my15}\begin{aligned}
    & J_{t,s}^\pi(x,z) \\  & = \textstyle \int_{C} \int_{S} \int_ {\mathcal{Z}} \cdots T_{\mu_{t-2}}\big( T_{\mu_{t-1}}(v_0^s)\big)(x_{t-2},z_{t-2}) \cdots \\ & \hphantom{==} \delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1) Q(\mathrm{d}x_1|x,u_{0}) \mu_{0}(\mathrm{d}u_{0}|x,z)
\end{aligned}\end{equation}
with $t-2$ copies of $C \times S \times \mathcal{Z}$ in \eqref{my15}. By repeating this process until the integral has only one copy of $C \times S \times \mathcal{Z}$, we conclude that
\begin{equation}\begin{aligned}
   & J_{t,s}^\pi(x,z) \\  & = \textstyle \int_{C} \int_{S} \int_ {\mathcal{Z}} T_{\mu_{1}}\big( \cdots \big( T_{\mu_{t-1}}(v_0^s)\big) \cdots \big)(x_{1},z_{1})  \\ & \hphantom{==} \delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1) Q(\mathrm{d}x_1|x,u_{0}) \mu_{0}(\mathrm{d}u_{0}|x,z)\\
   & = T_{\mu_{0}}( T_{\mu_{1}}( \cdots ( T_{\mu_{t-1}}(v_0^s) \cdots ) )(x,z),
\end{aligned}\end{equation}
where we use Def. \ref{DPoperator} to write the last line. Finally, if $t \in \mathbb{N}_0$ and $\pi = (\mu, \mu, \dots) \in \Pi$, then the previous result gives
\begin{equation}
    J_{t+1,s}^\pi(x,z) = T_{\mu}( T_{\mu} ( \cdots ( T_{\mu}(v_0^s) ) \cdots ))(x,z),
\end{equation}
where the operator $T_\mu$ is applied $t+1$ times. We write the outer-most $T_\mu$ using Def. \ref{DPoperator} to find that
\begin{equation}\begin{aligned}\label{almostthere}
   & J_{t+1,s}^\pi(x,z) \\ & = \textstyle \int_{C} \int_{S} \int_ {\mathcal{Z}} T_{\mu} \big( \cdots \big( T_{\mu}(v_0^s) \big) \cdots \big)(x_1,z_1) \delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1)\\ & \hphantom{==} Q(\mathrm{d}x_1|x,u_{0}) \mu(\mathrm{d}u_{0}|x,z),
\end{aligned}\end{equation}
where $t$ copies of $T_\mu$ appear explicitly in \eqref{almostthere}. Furthermore, $J_{t,s}^\pi(x_1,z_1)  = T_{\mu} \big( \cdots \big( T_{\mu}(v_0^s) \big) \cdots \big)(x_1,z_1)$, where $T_\mu$ is applied $t$ times. By substituting $J_{t,s}^\pi(x_1,z_1)$ into \eqref{almostthere}, we find that
\begin{equation}\begin{aligned}
     J_{t+1,s}^\pi(x,z) &  = \textstyle \int_{C} \int_{S} \int_ {\mathcal{Z}} J_{t,s}^\pi(x_1,z_1) \delta_{\max\{z,c(x,u_0)\}}(\mathrm{d}z_1)\\ & \hphantom{==} Q(\mathrm{d}x_1|x,u_{0}) \mu(\mathrm{d}u_{0}|x,z)\\
     & = T_\mu(J_{t,s}^\pi)(x,z),
\end{aligned}\end{equation}
where we use Def. \ref{DPoperator} to write the last line. 
%
%    Z_1(x_0,z_0,u_0,x_1,z_1,u_1,\dots) & = z_1 = \max\{z_0,c(x_0,u_0)\}\\
%    Z_2(x_0,z_0,u_0,x_1,z_1,u_1,\dots) & = z_2 = \max\{z_1,c(x_1,u_1)\} = \max\{z_0,c(x_0,u_0), c(x_1,u_1)\}\\
%$v_0^s(x,z) = \max\{ z-s,0\} = E_{x,z}^\pi(\max\{Z_0 - s,0\}) = J_{0,s}^\pi(x,z)$ for all $(x,z) \in S \times \mathcal{Z}$ and $\pi \in \Pi$.
%$J_{t,s}^{\pi^s}( y, q) = \underbrace{T_{\delta_{\kappa^s}}(  \cdots ( T_{\delta_{\kappa^s}}}_{t \text{ times}}(v_0^s) ) \cdots )(y,q)$ $\forall (y,q) \in S \times \mathcal{Z}$, and it follows that
%$J_{t+1,s}^{\pi^s}( x, z) =  \textstyle \int_C \int_S \int_{\mathcal{Z}} J_{t,s}^{\pi^s}( y, q) \delta_{\max\{z, c(x,u) \}}(\mathrm{d}q) Q(\mathrm{d}y|x,u) \delta_{\kappa^s(x,z)}(\mathrm{d}u)$.
\end{proof}
